TruthBot: An Automated Conversational Tool for Intent Learning, Curated Information Presenting, and Fake News Alerting

We present TruthBot, an all-in-one multilingual conversational chatbot designed for seeking truth (trustworthy and verified information) on specific topics. It helps users to obtain information specific to certain topics, fact-check information, and get recent news. The chatbot learns the intent of a query by training a deep neural network from the data of the previous intents and responds appropriately when it classifies the intent in one of the classes above. Each class is implemented as a separate module that uses either its own curated knowledge-base or searches the web to obtain the correct information. The topic of the chatbot is currently set to COVID-19. However, the bot can be easily customized to any topic-specific responses. Our experimental results show that each module performs significantly better than its closest competitor, which is verified both quantitatively and through several user-based surveys in multiple languages. TruthBot has been deployed in June 2020 and is currently running.

==> concl.tex <==
\section{Summary and Plans of Extension}
\label{sec:summary}

This paper provides a solution to social distancing using social scheduling and propose a mechanism that satisfies a lot of desirable theoretical properties. Experiments show that it is prioritizing users based on their urgency (at the cost of a cooling-off time) which the classical FCFS mechanism is unable to provide. It also reduces the rush-time congestion by a big proportion without dropping the customers. Convinced with the users interest in seeing this as an app, we have already started to develop the app that implements \mech.

% \sn{we should mention that the check of agents visiting the right slot can be used by the shop/facility owner. the users might be given a unique slot OTP which needs to match that of the shopkeeper and only then purchase can proceed (assuming shopkeepers also worry about their health and want to keep social distancing). for missed slots, we can assume the periods to be short, maybe 1-2 hours, so if someone misses a slot, he can participate in the next available scheduling -- OTP will ensure that he hasn't visited, hence his delay can be refunded.}



==> experiment.tex <==
\section{Experiments}
\label{sec:experiment}

While \mech\ satisfies several desirable properties of a social scheduling mechanism, its prioritizing profile for different classes of urgency, costs of prioritization, reduction in social congestion, scalability, and user explainability are not theoretically captured. This is why an experimental study is called for. 

For the experiments, we consider three discrete levels of valuations of the agents denoted by 3, 2, and 1, which can be interpreted as {\tt urgent}, {\tt medium}, and {\tt not-urgent} respectively. The numbers represent the agent's valuation if they are allocated their most preferred slot. The valuations for the other slots are assumed to decrease with a multiplying factor $\delta \in (0, 1)$ in the order of their slot preference, i.e., the valuation for the $t$-th most preferred slot of a {\tt medium} agent will be $2 \delta^{t-1}$. All optimizations used the Gurobi solver~\citep{gurobi} under an academic license.
% The agents in this setting are asked to report their slot preference order and what urgency their work is. 
% \sn{a little detailed overview of the section when it's complete}

\subsection{Prioritizing profile and its cost}
\label{sec:priority}

In this section, we investigate what are the typical priority slots allotted to an agent of a specific class in \mech. \Cref{fig:prioritization} shows the agents' allocated slot preferences (mean with one standard deviation) versus the population ($n$) plot where $m=5, k=4$, and $\delta=0.65$. The urgency of an agent is picked uniformly at random. Values of $n$ varies between $2$ to $1.1 mk$ in steps of 1 (for a population beyond $mk$ some agents have to be dropped). The experiment is repeated $10n$ times for every $n$. 
The top plot considers the case where every agent has an identical order of priority over the slots, while that of the bottom shows when agent's priorities are picked uniformly at random. 
The increase in the population increases the congestion, and it shows that the more urgent agents are given their more preferred slots in both the plots. However, when $n$ is small, i.e., there is little congestion, the difference in the preferences of their allocated slots are small.

Naturally, when the preferences are random, more agents can be allocated their more preferred slots since the most preferred slots of two individuals are less likely to be conflicting. This results in a significant overlap of the curves in the bottom plot. However, the conflicting nature grows with increase in the population. After all the slot capacities are exhausted (at $n=20$) the algorithm has to deny some agents. The mechanism denies only the {\tt not-urgent} agents and picks those that can be allocated a more preferred slot, which results in a downward slope in the {\tt not-urgent} curve. However, the upward trend of the other two classes continue.

The two plots in \Cref{fig:prioritization} show the two extreme cases (most conflicting to probabilistically least conflicting) of slot preferences of the agents. In practice, we are expected to see conditions that fall in between, though with a little bias towards the first case. This is because shoppers follow a general time-trend, e.g., evenings are generally a better shopping slot for all individuals.
% 
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{images/pref_pop_5_4_10_0.65_combined.pdf}
    \caption{Prioritization profile -- identical (top) and random (bottom) slot preferences}
    \label{fig:prioritization}
\end{figure}

However, \mech\ does the prioritized allocations of the agents at the cost of their delays. \Cref{fig:priority-delay} shows the plot of the priority of the allocated slot and the corresponding delays decided by \mech\ for each of these three classes. The parameters are chosen as before. The slot preferences of the agents are identical (to induce more congestion for a slot). The plot shows that an early slot allocation of an agent because of her urgency also comes with a longer delay, and shows the trade-off between these two decisions.

% When the slot preferences of the agents are picked uniformly at random, the allocated slot preferences of different classes are close to each other, and the payments are also significantly low (Fig. 4).
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{images/time_pop_5_4_10_0point65.pdf}
    \caption{Priority-delay trade-off}
    \label{fig:priority-delay}
\end{figure}


\subsection{Reduction in the social congestion}
\label{sec:reduction}

In this section, we consider real data of customer footfall in a general store that we have collected from the store. The raw dataset is available in the supplementary materials. The dataset contains the checkout (billing) time of the customers within from 7AM to 9PM (opening hours of the store) for the whole month of July 2020. Since the dataset was anonymized of customer identification, we have assumed that the billing timestamps are of unique users for a day. The approximate dimension of the store is $30 \times 30$ square-feet. With 6 feet being the minimum distance for a safe social distancing, the recommended number of people in the store at any time should roughly be 16 at any given time. If every shopper takes roughly 30 minutes to shop (including billing and checkout), then in an hour, the safety limit is 32 people an hour. However, the raw data shows that the average hourly population of the store was much above this, particularly during the rush hours (5-8PM) and on weekends -- the monthly average during the periods 5-6PM, 6-7PM, and 7-8PM were  38.00, 48.63, and 52.83 respectively. However, the monthly average of the population in an hour is 26.5, which is very much within the safety limits if social scheduling was implemented. Therefore, this dataset works as a perfect example where users can benefit greatly via social scheduling.

We divide the store opening hours into 14 hourly slots between 7AM to 9PM. Under \mech, the schedules are decided for a day. If a user is not allocated a slot on a certain day, she is given an option to update her urgency and preferences for the next day. For the experiments, we assume that the user increases the urgency increased by one level, e.g., {\tt not-urgent} becomes {\tt medium}, and keeps the slot preferences same. After three consecutive days if an agent is not allocated, she is considered `non-allocated' and alternative arrangements (e.g., home delivery) are made. \Cref{fig:congestion} shows the comparison of the average current population with that allocated by \mech\ for slot capacities of 24 (above) and 30 (below). The figures also show the non-allocated population in red. The figures show the trade-off between better social distancing and its cost (e.g., for home delivery). However, in both these cases the social congestion is reduced by approximately 50\% during the rush hours.
% 
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/congestion_24_30}
    \caption{Social congestion reduction, slot capacities $24$ (top) and $30$ (bottom)}
    \label{fig:congestion}
\end{figure}


\subsection{Scalability}
\label{sec:scalability}

 In this section, we examine \mech' computation time for finding the allocation and delays for a realistic population. We run \mech\ in \textsf{Python} for different number of slots ($m$) with slot capacity ($k$) being 12. For every $m$, we fixed $n = mk$ and repeated the experiment $10n$ times. \Cref{fig:scalability} shows the growth of the computation time of the mechanism. As a reference, to solve the allocation and delays for the store of \Cref{sec:reduction}, it takes about 100 secs. 
The simulations have been performed in a 64-bit Ubuntu 18.04 LTS machine with Intel(R) Core(TM) i7-7700HQ CPU @2.80GHz quad-core processors and 16 GB RAM.
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/scalability}
    \caption{Computation times of \mech}
    \label{fig:scalability}
\end{figure}


\subsection{Comparison with other scheduling mechanisms}
\label{sec:fcfs}

Since \mech\ is unique in the context of social scheduling for congestion management, there is no perfect comparison candidate. The closest scheduling applications are designed to help the customers book a slot for businesses. These apps book the slots using an FCFS protocol. In this section, we investigate if the population having the three classes of urgency appear randomly to the FCFS protocol, how they can be {\em misprioritized}. To quantitatively capture this effect, we define mispriority of an allocation $A$ as
\begin{align}
    \label{eq:mispriority}
    \textsf{misp}(A) &= \sum_{i \in N} \sum_{j \in N} \mathbb{1} (\rho_j(A) > \rho_i(A) \text{ and } \text{urg}_j > \text{urg}_i) \nonumber \\ & \cdot ((\rho_j(A) - \rho_i(A)) + (\text{urg}_j - \text{urg}_i) ).
\end{align}
Here $\rho_i(A)$ denotes the allocated slot preference of $i$ under $A$ and urg$_i$ denotes the urgency of $i$. The metric therefore finds the cases where a more urgent agent is allocated a less preferred slot than a less urgent agent and weights that case with the amount of difference in the urgency and their difference in allocated slot preferences. Clearly, if a more urgent agent is always provided a more preferred slot, then this metric will yield zero for that allocation policy.

We run the FCFS protocol for $n$ agents with both their urgency and order of arrivals chosen uniformly at random. We repeat this experiment $10n$ times for every $n$. \Cref{fig:mispriority} shows the mispriority of the FCFS protocol when $m=5,k=4$ and $n$ is varied from $2$ to $1.1 mk$ in steps of 1. It shows that the increase in congestion also increases the mispriority of the FCFS protocol.
% 
Since \mech\ prioritizes the users according to their urgency by design, mispriority will always be zero for it.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/mispriority_5_4_10_FCFS.pdf}
    \caption{Misprioritization of FCFS}
    \label{fig:mispriority}
\end{figure}


\subsection{User comprehension and acceptability survey}
\label{sec:survey}

To understand if the mechanism is easy for the users to comprehend or not, we ran a survey on the usual customers of the store of \Cref{sec:reduction}. A total of 57 users participated in this survey. We explained the details of \mech\ along with a few examples and asked them the following questions: (1)~should social scheduling be done based on users’ urgency? (2)~are they convinced that \mech\ prioritizes based on users’ urgency? (3)~whether prioritized allocation coming with a longer delay is fair for users of different urgency? (4)~does FCFS capture the urgency of users’ needs? (5)~is \mech\ superior to FCFS on the need-based priority aspect? (6)~does \mech\ maintain the recommended capacity of a store at any time for social distancing norms? (7)~do they want to see a mobile app that implements \mech\ for the users?

\Cref{fig:survey} shows that the users could comprehend the salient features of this mechanism and accept to have this mechanism implemented as an app. The survey response data is also submitted as supplementary material.
\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{images/survey_plot.pdf}
    \caption{User survey}
    \label{fig:survey}
\end{figure}


% \sn{points to be discussed in this section (with experimental results)}
% \begin{enumerate}
%     \item description of the experimental setup -- for synthetic and real data experiments
%     \item prioritizing profile and its cost. priorities for different classes -- when the slot preferences are random for different agents. the corresponding delays should also be added.
%     \item reduction in social congestion. how would the congestion be if everyone took a random decision to visit a facility.
%     \item scalability. simulate with large m and n.
%     \item real movement data. the previous three points above to be done again on it.
%     \item in each of the cases before, how would it be compared to other mechanisms? what are good candidates for comparison?
%     \item human subject experiment. need to think about it a bit. e.g., what do they think about the fairness, equal opportunity to all, prioritize based on need, and foolproofness? this could be a survey after they use the app or view outputs. physical visit may be necessary since this is the real human subject study.
% \end{enumerate}
% \sn{end points}



==> intro.tex <==
\section{Introduction}
\label{sec:intro}

Pandemics like COVID-19 showed that the most effective solution against infectious diseases is {\em social distancing} until a reliable vaccine is found \citep{smith20}. Therefore, it is a practice we ought to master and stay prepared as a preventive disease containment measure in future. While citizens are willing to follow social distancing, the lack of communication and coordination among them, particularly prior to an immediate lockdown, overcrowds shopping centers even though the footfalls could have been evenly distributed over the working hours of the shop to maintain a recommended social distance. 
% 
This setting is different from rostering staff in organizations, since in such settings the requirement of staff determine their slots and they are not distinguished on urgency. Also, the organization can enforce the movements according to a roster. However, in our setting the customers have different levels of urgency and independently decide their own moves. We assume that they are {\em rational}, i.e., along with their urgency they are also concerned with their health safety and want to maintain a social distance.

In this paper, we introduce \mech\ (\mechfull) which solves this social coordination problem with the help of {\em mechanism design}. The mechanism is run for a facility that has a recommended maximum footfall (the {\em capacity}) for a duration of time (a {\em slot}) to maintain social distance. Unlike various other appointment maintaining apps, \mech\ takes inputs from all users willing to visit the store and schedules them according to their urgency and slot preferences. Apart from this, the algorithm is also capable of (a) ensuring that the users do not overstate (or understate) their urgency, (b) maintaining voluntary participation of the users, and (c) scheduling at large scale for large number of users and store capacity in a computationally tractable manner. \mech\ puts together concepts of economic theory and optimization to deliver all these properties.

To our knowledge, this is the first of its kind application of game theory to pandemic containment by reducing the congestion in facilities that satisfies such desirable theoretical properties and exhibit fair and truthful handling of the individuals of different urgency. The following section details the contributions of this paper with references to the theoretical and experimental results.


\subsection{Brief Problem Description and Contributions}
\label{sec:contributions}

% We propose a mechanism that decides the schedule of the visit of all the individuals of a facility. 
The opening hours of the facility is divided into {\em periods}, each of which have multiple {\em slots}. The customers report their valuations over these slots in a period. A valuation $v_{ij}$ reflects how many slots $i$ is willing to wait before accessing the facility again if she is allocated slot $j$. A higher valuation indicates that the agent is in a higher urgency to get that slot. The valuations of a customer (agent) are represented a vector of real numbers, whose length is the number of slots in that period. A social scheduling mechanism takes these reports and allocates the slots in that period and also decide a delay until which an agent cannot access the facility. Quite naturally, an agent prefers to have a more preferred slot assigned to her with less delay.
This competitive scenario induces a {\em game}\footnote{A {\em game} is a strategic interaction between multiple self-interested agents.} where agents' actions are to report the valuations. The agents may {\em overstate} (or {\em understate}, both of which are different from truthtelling) their actual valuations.

We model the payoffs of the agents using the well-known quasi-linear payoff model \cite[Chap 10]{SL08} and propose \mech, which decides the allocation and delay in every period of this game. The allocation ensures that each slot admits a maximum number of agents maintaining the social distancing norms.
\begin{itemize}
    \item Our first result (\Cref{thm:dsic}) shows that (a)~the allocation of \mech\ maximizes the sum of the valuations of the agents, and (b)~the best response of the agents will be to report their urgency {\em truthfully} to the decision maker. Later in \Cref{sec:priority}, we show that this allocation can be interpreted as that the agents having a higher urgency will be allocated more preferred slots. The widely used FCFS slot booking mechanism cannot satisfy this property (\Cref{sec:fcfs}).
    \item The next result (\Cref{thm:ir}) shows that the net payoff of an agent from participating in \mech\ is always non-negative, which implies that the agent will be weakly better off by participating in the mechanism.
    \item Even though the optimization problem of \mech\ falls in the class of {\em integer programs}, which is computationally intractable in general, we show in \Cref{thm:relax,thm:strong} that there exists a {\em strongly polynomial} relaxed problem which is sufficient to reach the optimal solution.
    \item Experiments in \Cref{sec:priority} show that prioritization comes at the cost of a higher delay, which also exhibit the tradeoff between expedited allocation and delay. \Cref{sec:reduction} considers the data of normal footfall in a general store and shows that the introduction of \mech\ can reduce the congestion by about 50\% on an average during the busy hours of the day without dropping any customer overall. Finally, we run a survey to understand the explainability and user acceptance of \mech\ (\cref{sec:survey}).
\end{itemize}

\subsection{Related Work}
\label{sec:literature}

Social distancing measures have been widely successful and recommended for pandemic control \citep{glass2006targeted,thunstrom2020benefits,fong2020nonpharmaceutical}. However, it is also observed that the benefits of social distancing depend on the extent to which it is used by the citizens. Individuals are sometimes reluctant to pay the costs inherent in social distancing, and this can limit its effectiveness as a control measure \citep{reluga2010game}. This is particularly important when the movement of the people are largely non-coordinated. Coordination is essential for social distancing \citep{shadmehr2020coordination}, but the technology is still not much developed to address the social coordination problem, particularly when the participants are self-interested independent decision makers. An artificially intelligent app can help them in coordinating, but to design it on the face of the strategic behavior of the participants poses a challenge.

A related thread of social distancing measures exist in workforce-intensive organizations in the forms of rostering, workplace design, allowing people to work from home~\citep{roycroft2020rostering}. However, these measures are centrally controlled and an individual does not have a scope to behave strategically.

The businesses, on the other hand, maintain social distancing by enforcing certain appointment booking apps (either web or smartphone-based) to their customers. These apps run a {\em first-come-first-served} (FCFS) algorithm for slot booking, and does not provide any priority preservation guarantees.\footnote{An example app is \url{www.appointy.com}.}

Resource allocation is a related problem where a lot of game theoretic ideas have been used in the literature. For instance, cloud computing~\citep{nezarat2015efficient}, grid computing~\citep{khan2006non}, wireless networks~\citep{zhou2014auction}, and many more application domains use ideas from game theory and auction theory. However, all of these methods involve monetary transfer as these application domains admit options of transferring money.

Our problem formulation and its solution is unique in the sense that we use time as a replacement of money in the context of pandemic containment. While social distancing is a highly desirable coordinated effort, charging money to do the same is perhaps unethical and unacceptable in many countries. However, waiting time is often seen as a resource that individuals agree to trade with \citep{leclerc1995waiting}. 

% The paper is organized as follows. \Cref{sec:setup} describes the basic setup of the problem and introduces the notation. \Cref{sec:desiderata} introduces the desirable theoretical properties, \Cref{sec:online} introduces the central mechanism of the paper, and \Cref{sec:theory} proves its theoretical properties. \Cref{sec:experiment} discusses the detailed experiments other aspects of this mechanism that are not directly captured in the theoretical analysis. We conclude the paper in \Cref{sec:summary}.

==> model_theory.tex <==
\section{Problem Setup}
\label{sec:setup}

Define $N \coloneqq \{1, \ldots, n\}$ to be the set of agents that are trying to access a facility ${\cal F}$. Time is divided into {\em periods}, and each period is further divided into {\em slots}. The set of slots is denoted by $M \coloneqq \{1, \ldots, m\}$. Every slot has a maximum capacity of $k$, which is decided by the social distancing norm of the region and the size of the facility. A {\em central planner} (e.g., an AI app) allocates these slots to the agents maintaining the capacity constraint. Every agent has a preference over the slots which is represented by a real number against each slot. For instance, the preference (we will call this the agent's {\em valuation}) of agent $i$ for slot $j$ is denoted by $v_{ij} \in \mathbb{R}_{\geqslant 0}$, which is interpreted as if slot $j$ is allotted to $i$, then $i$ is willing to wait for $v_{ij}$ time periods before requesting another access to the facility.\footnote{The valuation $v_{ij}$ need not be integral. In practice, the facility will be frozen for that duration of time in the booking app.} Thus the valuation implicitly reflects the urgency to visit the facility for that agent. 
% An example framework for such urgency representation could be to assign finite levels of urgency -- \texttt{urgent, medium, not-urgent} -- and assign fixed numbers for them. 
The valuation vector of $i$ is represented by $v_i \in \mathbb{R}_{\geqslant 0}^m$.
% 
In this paper, we consider different facilities independently.
The joint facility slot allocation problem can be modeled as a similar problem with the additional constraint that the same slot cannot be allocated to the same agent at different facilities. We leave the detailed analysis for it as a future work.

The planner decides the allocation which can be represented as a matrix $A = [a_{ij}]$, where $a_{ij} = 1$, if agent $i$ is allotted slot $j$, and zero otherwise. We assume that every agent can be assigned at most one slot in a period. We denote the slot assigned to $i$ by $a_i^*$. The planner also decides a delay $d = (d_i, i \in N)$ for each agent before which they cannot make another request to the system. We assume that every agent wants a more valued slot to be assigned to her and also wants to wait less. Therefore, the net payoff of an agent is assumed to follow a standard {\em quasi-linear form}~\citep{SL08}
\begin{equation}
    \label{eq:utility}
    u_i((A,d), v_i) = v_i(A) - d_i, \text{ where } v_i(A) = v_{i a_i^*}.
\end{equation}
Denote the set of all allocations by ${\cal A}$ and $d_i \in \mathbb{R}, \forall i \in N$. The planner does not know the valuations (or urgencies) of the agents. Therefore he needs the agents to report their valuations and decide the allocation and the delay. This leaves the opportunity for an agent to misrepresent her true valuation, e.g., an agent can report a \texttt{not-urgent} valuation as \texttt{urgent} for a prioritized scheduling. To distinguish, we use $v_{ij}$ for the true valuation and $\hat{v}_{ij}$ for reported valuations. We will use the shorthand $v = (v_i)_{i \in N}$ to denote the true valuation profile represented as an $m \times n$ real matrix, and $\hat{v}$ to denote the reported valuation profile. The notation $v_{-i}$ denotes the valuation profile of the agents except $i$.
% 
The decision problem of the planner is therefore formally captured by the following function.
\begin{definition}[Social Scheduling Function (SSF)]
 A {\em social scheduling function (SSF)} is a mapping $f : \mathbb{R}^{m \times n} \to {\cal A} \times \mathbb{R}^n$ that maps the reported valuations to an allocation and delay for every agent. Hence, $f(\hat{v}) = (A(\hat{v}), d(\hat{v}))$, where $A$ is the allocation and $d$ is the delay function.\footnote{We overload the notation $A$ and $d$ to denote both functions and values of those functions, since their use will be clear from the context.}
\end{definition}



% \sn{need to say something more}

\section{Design Desiderata}
\label{sec:desiderata}

In this section, we formally define a few desirable properties that a social scheduling algorithm should satisfy. The properties address the issues of prioritization, truthfulness, voluntary participation, and computational complexity.

The first property ensures that the allocation is {\em efficient} in each period, i.e., it maximizes the sum of the valuations of all the agents. As an effect, every slot will be allocated to an agent who values it the most, breaking ties arbitrarily.
\begin{definition}[Efficient Per Period (EPP)]
 \label{def:efficiency}
 An SSF $f$ is {\em efficient per period (EPP)} if at every period, it chooses an allocation $A^*$ that maximizes the sum of the valuations of all the agents. Formally, if $f(\cdot) = (A^*(\cdot), d(\cdot))$, then for every $v$
 \begin{equation}
     \label{eq:efficient}
     A^*(v) \in \argmax_{A \in {\cal A}} \sum_{i \in N} \sum_{j \in M} v_{ij} a_{ij}.
 \end{equation}
\end{definition}

However, since the planner can only access the reported values $\hat{v}_i$'s which can be different from the true $v_i$'s, it is necessary that the reported values are indeed the true values. The following property ensures that the robots are incentivized to `truthfully' reveal these information.
\begin{definition}[Per Period Dominant Strategy Truthful]
 \label{def:non-manipulability}
 An SSF $f(\cdot) = (A(\cdot), d(\cdot))$ is {\em truthful in dominant strategies per period} if for every $v_i, \hat{v}_i, \hat{v}_{-i}$, and $i \in N$
  \begin{align*}
   v_i(A(v_i, \hat{v}_{-i})) - d_i(v_i, \hat{v}_{-i}) \geqslant v_i(A(\hat{v}_i, \hat{v}_{-i})) - d_i(\hat{v}_i, \hat{v}_{-i}).
  \end{align*}
\end{definition}
The inequality above shows that if the true value of agent $i$ is $v_i$, the allocation and delay resulting from reporting it `truthfully' maximizes her payoff {\em irrespective of the reports of the other robots}.

\begin{definition}[Individual Rationality]
 \label{def:ir}
 An SSF $f(\cdot) = (A(\cdot), d(\cdot))$ is {\em individually rational} if for every $v$, and $i \in N$
  \begin{align*}
   v_i(A(v)) - d_i(v) &\geqslant 0.
  \end{align*}
\end{definition}
Individual rationality ensures that it is always weakly beneficial for every rational agent to participate in such a mechanism.

In large facilities, the number and capacities of the slots are large, and this leads to an exponential increase in the size of the set ${\cal A}$. In an online setting, where the allocations and delays have to be decided quickly, it is desirable to have an SSF that is computable in a time polynomial in $n$ and $m$. We consider algorithms that are {\em strongly polynomial}. Strongly polynomial algorithms are defined by their arithmetic model of computation. The basic arithmetic operations (addition, subtraction, multiplication, division, and comparison) take a unit time step to perform, regardless of the sizes of the operands. 

% [refer to the wikipedia article: https://en.wikipedia.org/wiki/Time_complexity#Strongly_and_weakly_polynomial_time]

\begin{definition}[Strongly Polynomial]
 \label{def:strong-poly}
    An algorithm runs in {\em strongly polynomial time} if \citep{grotschel1993complexity}
    \begin{itemize}
        \item the number of operations in the arithmetic model of computation is bounded by a polynomial in the number of operands in the input instance; and
        \item the space used by the algorithm is bounded by a polynomial in the size of the input.
    \end{itemize}
\end{definition}



% \sn{need to say a few words}


\section{Periodic Mechanisms}
\label{sec:online}

We consider mechanisms that run at every period of this social scheduling problem. The agents report their valuations in the beginning of every period. The planner decides the schedules and delays.\footnote{For mechanisms that consider the finite or infinite horizon of such allocation problems \citep[e.g.]{bergemann-valimaki10dynamic-pivot}, (a)~the designer needs to know the transition probabilities, (b)~solution concepts are weaker, and (c)~are computationally expensive. These factors made us restrict our attention to periodic mechanisms.}

% \footnote{In a practical implementation, the decision might be taken one or two periods before since that provides the agents some time to be prepared.}

In our setting, the agents have the opportunity to overstate their urgencies to get a better slot allotted to them. This is precisely where our approach using the ideas of mechanism design \citep{borgers2015introduction} is useful. 

 In a setting where the agents' valuations are private, if the mechanism has no additional tool (e.g., delays in time in our context) to penalize overstating, only {\em dictatorial} mechanisms (where a pre-selected agent's favorite outcome is selected always) are truthful \citep{Gib73,Sat75}. This negative result holds irrespective of whether agents' preferences are {\em ordinal} (representable as an order relation over the outcomes) or {\em cardinal} (agents have a real number to represent the intensity of the preference). Note that in our setup, the agents' preferences are cardinal.
 A complementary analysis by \citet[Thm 7.2]{Roberts79} shows that a dictatorship result reappears under certain mild conditions in a {\em quasi-linear} setting (which is our current setting), unless transfers (of utility) are allowed. 
%  Transfers, in these settings, is used as a means of transferring value from an agent to another, and it is shown to help by unraveling the true values of the agents. 
 In this paper, we use delay as a surrogate for transferable utility among the agents to ensure truthful value revelation at every period. 
 
We are now in a position to present the proposed mechanism \mech\ (\mechfull).

\subsection{Description of \mech}

The SSF needs to decide on the allocation $A$ and the delay $d$. The actual allocation that satisfies EPP is given by the following integer program (IP).
\begin{align}
 \label{eqn:IP}
 \begin{split}
     \argmax_{A} & \sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij} \\
     \text{s.t. } & \sum_{j \in M} a_{ij} \leqslant 1, \ \forall i \in N, \\
     & \sum_{i \in N} a_{ij} \leqslant k, \ \forall j \in M, \\
     & a_{ij} \in \{0, 1\}, \ \forall i \in N, j \in M.
 \end{split}
\end{align}
However, IPs are NP-complete in general. Therefore, \mech\ computes the LP relaxation of the above problem, given as follows.
\begin{align}
 \label{eqn:LP}
 \begin{split}
     \argmax_{A} & \sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij} \\
     \text{s.t. } & \sum_{j \in M} a_{ij} \leqslant 1, \ \forall i \in N, \\
     & \sum_{i \in N} a_{ij} \leqslant k, \ \forall j \in M, \\
     & a_{ij} \geqslant 0, \ \forall i \in N, j \in M.
 \end{split}
\end{align}
We will show that this is without loss of optimality, since the solution to LP~\ref{eqn:LP} will always be integral and will coincide with the solution of IP~\ref{eqn:IP}. 

The delay of agents are computed via the standard Vickery-Clarke-Groves (VCG) rule \citep{Vick61,Clar71,Grov73}. Denote the optimal allocation of LP~\ref{eqn:LP} by $A^*(v)$. Also, denote the allocation given by LP~\ref{eqn:LP} when agent $i$ is removed from the system by $A^*_{-i}(v_{-i})$.
% 
For agent $i$, the delay is given by,
\begin{align}
\label{eqn:payment}
\begin{split}
    d_i &:= \sum_{\ell \in N \setminus \{i\}} v_\ell(A^*_{-i}) - \sum_{\ell \in N \setminus \{i\}}  v_\ell(A^*). 
\end{split}
\end{align}
The mechanism in every period is described in \Cref{algo:collision}.

\begin{algorithm}[t!]
 \caption{\mech\ in every period}
 \begin{algorithmic}[1]
   \STATE {\bf Input:} for every agent $i \in N$, the value $\hat{v}_i$
      \STATE compute $A^*(\hat{v})$ (\Cref{eqn:LP}) as the allocation \label{alg:allocation-step}
      \STATE charge a delay $d_i(\hat{v})$ (\Cref{eqn:payment}) to every $i \in N$ for which they cannot access the scheduling mechanism again
    \STATE {\bf Output:} $A^*(\hat{v})$ and $d(\hat{v})$
  \end{algorithmic}
 \label{algo:collision}
 \end{algorithm}

Note that the allocation is different from that of a sorted urgency sequential dictator, i.e., where the agents are sorted based on their urgency and asked to pick their favorite slots in that order. For example, consider two agents A and B, and two slots of capacity one. Valuations are (51, 50) and (50, 0) respectively for A and B respectively for the two slots -- sequential dictator would allocate slot 1 to A and 2 to B, while the socially optimal is to allocate slots 2 and 1 to A and B respectively, which is allocated by \mech.

\section{Theoretical guarantees}
\label{sec:theory}


Our first result shows that \mech\ ensures proper prioritization of the agents and reveals their urgency truthfully.
\begin{theorem}
\label{thm:dsic}
 \mech\ is EPP and per period dominant strategy truthful.
\end{theorem}


% \shortversion{\noindent \mech\ is EPP by construction. This proof of per period dominant strategy truthful is a standard extension of the proof for Vickery-Clarke-Groves (VCG) mechanism \citep{Vick61,Clar71,Grov73} and is skipped here.
% }

% \longversion{
\begin{proof}
 \mech\ is EPP by construction. Hence, we only prove that it is per period dominant strategy truthful. This proof is a standard exercise in the line of the proof for Vickery-Clarke-Groves (VCG) mechanism \citep{Vick61,Clar71,Grov73}. The payoff of agent $i$ is
% \begin{gather}
 \begin{align*}
   \lefteqn{ v_i(A^*(v_i, \hat{v}_{-i})) - d_i(v_i, \hat{v}_{-i})} \\
   &= \left( v_i(A^*(v_i, \hat{v}_{-i})) + \sum_{j \in N \setminus \{i\}}  \hat{v}_j(A^*(v_i, \hat{v}_{-i})) \right) - \sum_{j \in N \setminus \{i\}} \hat{v}_j(A^*_{-i}) \\
   &\geqslant \left( v_i(A^*(\hat{v}_i, \hat{v}_{-i})) + \sum_{j \in N \setminus \{i\}}  \hat{v}_j(A^*(\hat{v}_i, \hat{v}_{-i})) \right) - \sum_{j \in N \setminus \{i\}} \hat{v}_j(A^*_{-i}) \\
   &= v_i(A^*(\hat{v}_i, \hat{v}_{-i})) - d_i(\hat{v}_i, \hat{v}_{-i}).
  \end{align*}
% \end{gather}
The first equality is obtained by writing and reorganizing the expression for $d_i$. The inequality holds since by definition $\sum_{j \in N}  v_j(A^*(v_i, \hat{v}_{-i}), \hat{v}_j) \geqslant \sum_{j \in N}  v_j(A, \hat{v}_j)$ for every $A$; in particular, we chose $A^*(\hat{v}_i, \hat{v}_{-i})$. The last equality is obtained by reorganizing the expressions again.
\end{proof}
% }

The next result ensures that the agents are incentivized to voluntarily participate in \mech.
\begin{theorem}
 \label{thm:ir}
 \mech\ is individually rational for every agent.
\end{theorem}

\begin{proof}
 Consider agent $i$. The utility of $i$ under \mech\ is given by
 \begin{align*}
     \lefteqn{ v_i(A^*(v)) - d_i(v) } \\
     &= v_i(A^*) - \left( \sum_{\ell \in N \setminus \{i\}} v_\ell(A^*_{-i}) - \sum_{\ell \in N \setminus \{i\}}  v_\ell(A^*) \right) \\
     &= \left( \sum_{\ell \in N}  v_\ell(A^*) - \sum_{\ell \in N} v_\ell(A^*_{-i}) \right) + v_i(A^*_{-i}) \geqslant 0
 \end{align*}
 The second equality holds by reorganizing the terms and by adding and subtracting $v_i(A^*_{-i})$. Note that the difference term in the parentheses in the last expression is always non-negative since $A^*$ is the optimal allocation for all allocations. In particular, $A^*_{-i}$ is also a feasible allocation when agent $i$ is present. The term $v_i(A^*_{-i})$ is zero. Hence the inequality follows.
\end{proof}

The next few results show that even if the allocation problem of IP~\ref{eqn:IP} falls in a computationally intractable class, its special structure can be used to find a tractable solution.
\begin{theorem}
 \label{thm:relax}
 The allocation of \mech\ given by LP~\ref{eqn:LP} always gives integral solutions.
\end{theorem}

\begin{proof}
 Consider the vector $x^\top = (a_{11}, \ldots, a_{1m}, \ldots, a_{n1}, \ldots, a_{nm})$, i.e., the rows of $A$ linearized as a vector. We can write the constraints of LP~\ref{eqn:LP} in using a $(n+m) \times nm$ constraint matrix, s.t.,
 \[
 \left ( 
 \begin{array}{ccccccccc}
     1 & \ldots & 1 & 0 & \ldots & 0 & 0 & \ldots & 0 \\
     0 & \ldots & 0 & 1 & \ldots & 1 & 0 & \ldots & 0 \\
     &&&&\ldots&&&& \\
     1 & \ldots & 0 & 1 & \ldots & 0 & 1 & \ldots & 0 \\
     0 & 1 & \ldots & 0 & 1 & \ldots & 0 & 1 & 0 \\
     &&&&\ldots&&&&
 \end{array}
 \right ) x \leqslant \left ( \begin{array}{c}
     1 \\
      \vdots \\
      k \\
      \vdots
 \end{array}\right )\]
 Denote the matrix on the LHS by $C$. The first $n$ and the next $m$ rows correspond to the first and second set of constraints of LP~\ref{eqn:LP} respectively. We show that $C$ is totally unimodular (TU), which is sufficient to conclude that LP~\ref{eqn:LP} has integral solutions.
 We use the Ghouila-Houri characterization \citep{camion1965characterization} to prove that $C$ is TU. According to this characterization, a $p \times q$ matrix $C$ is TU if and only if each set $R \subseteq \{ 1,2, \cdots, p\}$ can be partitioned into two sets $R_1$ and $R_2$, such that, $\sum\limits_{i \in R_{1}} a_{ij} - \sum\limits_{i \in R_{2}} a_{ij} \in \{ 1,0,-1\}$, for $j= 1,2,\cdots,q$. Note that, in $C$ every column has two 1's, one in the first $n$ rows and one in the next $m$ rows. Pick any subset $R$ of the rows, construct the $R_1$ to be the rows that come from the first $n$ rows, and $R_2$ to be the rows that come from the last $m$ rows (one of these partitions can be empty). Clearly, the difference in each column of the rows $R$ will lie in $\{1,0,-1\}$. Hence proved.
\end{proof}

The result above shows that the solution to the LP relaxation of the allocation problem is without loss of optimality. LPs are known to be polynomially computable. However, in general it can be weakly polynomial, i.e., the space used by the algorithm may not be bounded by a polynomial in the size of the input. The forthcoming results show that the solutions of allocation and delays of \mech\ are strongly polynomial (\Cref{def:strong-poly}). 
To show this, we will first reduce the allocation problem (LP~\ref{eqn:LP}) to a minimum weight $b$-matching problem, which is known to be strongly polynomial \citep{schrijver2003combinatorial}.

Consider an edge-weighted bipartite graph $(N, M, E)$, where $N$ and $M$ are the agent set and set of slots respectively. The set $E$ denotes the edges $(i,j)$ with weights $-v_{ij}$. The matching constraints given by $b_i = 1, \forall i \in N$, and $b_j = k, \forall j \in M$.

\begin{lemma}
\label{lem:equivalence}
 Let $E^* \subseteq E$ be a perfect $b$-matching in $(N, M, E)$ and $A^* = [a_{ij}^*]_{i \in N, j\in M}$ be an allocation where $a_{ij}^* = 1 \Leftrightarrow (i,j) \in E^*$. The matching $E^*$ is a minimum weight perfect $b$-matching iff $A^*$ is an optimal solution to LP~\ref{eqn:LP}.
\end{lemma}

\begin{proof}
 We prove this via contradiction. Suppose $A^*$ is not an optimal solution to LP~\ref{eqn:LP}, i.e., there exists $A'$ which satisfies the constraints and yet gives a larger value to the objective function than that of $A$. Hence, $\sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij}' > \sum_{j \in M} \sum_{i \in N} v_{ij} a_{ij}^*$. Consider the edge set $E'$ corresponding to $A'$. Clearly this is a perfect $b$-matching, since $A'$ satisfies the constraints of LP~\ref{eqn:LP}, and $E'$ gives a lower weight than $E^*$, which proves that $E^*$ is not the minimum weight perfect $b$-matching. The implications can be reversed to obtain the other direction of the proof.
\end{proof}
Note that the delays are calculated by solving an equivalent LP like LP~\ref{eqn:LP} with one less agent. Each of these LPs is therefore strongly polynomial and the planner needs to solve $n$ of them. The computation of the each delay needs addition of $2(n-1)$ terms and one subtraction. Hence, the number of computations is polynomial in the number of numbers in the input instance and the space required is polynomial in the size of the input. Therefore we conclude the following.

\begin{corollary}
\label{cor:delay}
 The computation of the delays in \mech\ is strongly polynomial.
\end{corollary}
Combining \Cref{thm:relax}, \Cref{lem:equivalence}, and \Cref{cor:delay},  we get the following result.

\begin{theorem}
 \label{thm:strong}
  \mech\ provides a combinatorial, strongly polynomial algorithm for computing a social schedule and delays.
\end{theorem}


In the following section, we investigate the performance of \mech\ in real-world scenarios.

